Multi Actor-Critic DDPG for Robot Action Space Decomposition: A Framework to Control Large 3D Deformation of Soft Linear Objects

Robotic manipulation of deformable linear objects (DLOs) has great potential for applications in diverse fields such as agriculture or industry. However, a major challenge lies in acquiring accurate deformation models that describe the relationship between robot motion and DLO deformations. Such models are difficult to calculate analytically and vary among DLOs. Consequently, manipulating DLOs poses significant challenges, particularly in achieving large deformations that require highly accurate global models. To address these challenges, this paper presents MultiAC6: a new multi Actor-Critic framework for robot action space decomposition to control large 3D deformations of DLOs. In our approach, two deep reinforcement learning (DRL) agents orient and position a robot gripper to deform a DLO into the desired shape. Unlike previous DRL-based studies, MultiAC6 is able to solve the sim-to-real gap, achieving large 3D deformations up to 40 cm in real-world settings. Experimental results also show that MultiAC6 has a 66\% higher success rate than a single-agent approach. Further experimental studies demonstrate that MultiAC6 generalizes well, without retraining, to DLOs with different lengths or materials.

==> discussion.tex <==
\section{Discussion}
The simulation and experimental results clearly emphasize the benefits of actuating the 6 DOF of a gripper. These results suggest that controlling the gripper orientation necessary but not sufficient to close the sim-to-real gap. By exploiting the gripper orientation within the MultiAC6 framework, the robot can achieve, with the same model, complex deformations for various DLOs. To do so, the desired orientation of the DLO tip $\boldsymbol{\zeta}$ is required to define the state of $\text{Agent}_o$. This may be impracticable for real-world deployment and could be related to many methods that require online fine-tuning \cite{Yu2023, Lagneau2020, Reza2022}. However, during our experiments, we noticed that MultiAC6 could accommodate coarse values of $\boldsymbol{\zeta}$ to achieve the desired DLo deformation. Taking advantage of the robustness of MultiAC6, the same orientation $\boldsymbol{\zeta}$ can be transferred to different DLOs without affecting real-world performance. Furthermore, these orientations $\boldsymbol{\zeta}$ can be defined in advance without accurate measurements. This may be less restrictive than online fine-tuning.

==> method_old.tex <==
\section{Components of our DRL framework} \label{Background}
In this section, we present standard components of DRL systems that we use in our framework. We focus on explaining how we incorporate them in the framework. The elements include the RL procedure, the Bellman equation, the DDPG algorithm, and the reward function. 

\begin{figure*}[ht]
\centering
    \includegraphics[width=\textwidth]{Rl_algo.jpg}
\caption{Overview of our proposed framework for controlling the deformation of a soft object via the DDPG algorithm. The structure of the full DRL system and relevant parameters are displayed.}
\label{Rl_algo}
\vspace{-5mm}
\end{figure*}

\subsection{RL procedure}
We consider a classical trial-and-error RL procedure consisting of an agent (e.g., robot) interacting with the environment (e.g., the soft object) based on the policy to maximize rewards on discrete timesteps\cite{Lillicrap2015DDPG}. In each transition $t$, the agent starts from the state $s_t$, and takes an action $a_t$, which changes the state to a next state $s^\prime_t$\cite{Zakaria2021Frontiers}. The state $s_t$ and the action $a_t$ are included in the continuous state space $\mathcal{S}$, and the continuous action space $\mathcal{A}$, respectively, i.e., $s_t \in \mathcal{S}$ and $a_t \in \mathcal{A}$.

The observation the agent got from the environment describes the changes that happened by moving from state $s_t$ to $s^\prime_t$. The reward $r_t$ evaluates the action taken $a_t$ according to the task goal. The agent's goal is to learn the optimal policy $\pi^*: \mathcal{S} \longrightarrow \mathcal{A}$ throughout the different transitions. A transition $t$ is made of an action $a_t$, a state $s_t$, a next state $s_t'$, and a reward $r_t$.

\subsection{Bellman equation}
The Bellman equation\cite{Nachum2017ANIPS} is used to calculate a Q-value $Q_{B_t}(s_t,a_t)$ that evaluates the action $a_t$ chosen in a current state $s_t$. The Bellman equation (\ref{bellman_equation}) considers the discount factor $(\gamma \in [0.9,1])$ and the next Q-values $Q^\prime_t(s^\prime_t,a^\prime_t)$ to calculate $Q_{B_t}(s_t,a_t)$. The discount factor controls how much the DRL learning is considering future rewards. The next Q-values  $Q^\prime_t(s^\prime_t,a^\prime_t)$ are calculated for choosing the next action $a^\prime_t$ in the next state $s^\prime_t$.
\begin{equation} \label{bellman_equation}
   Q_{B_t}(s_t,a_t) = r_t + \gamma \times Q^\prime_t(s^\prime_t,a^\prime_t).
\end{equation}


\subsection{Off-policy vs on-policy learning}
We choose to use an off-policy (as opposed to on-policy) algorithm because it allows parallelizing the learning\cite{Hausknecht2016AAAI}. Parallelizing the learning means executing multiple agents in parallel on various environment instances. The learning parallelization technique speeds up the convergence, i.e., learning can be faster\cite{Kretchmar2002CSCI, Clemente2017arXiv}. We will discuss this concept further in Section~\ref{parallelization}.

\subsection{Deep Deterministic Policy Gradient (DDPG)}
The DDPG is a DRL algorithm based on Actor-Critic methods used for dealing with continuous action spaces\cite{Lillicrap2015DDPG}. It learns a Q-function and a policy by utilizing off-policy data and the Bellman equation\cite{Jangir2020ICRA}. The actor network (policy network) has as input the state $s_t$ and gives as output the optimal action $a_t$. The critic network (Q-function network) evaluates the optimality of the action $a_t$ chosen at state $s_t$ by attributing it the Q-values $Q_t(s_t,a_t)$ at transition $t$. Figure~\ref{Rl_algo} presents an overview of the framework established to make the robot deform a soft object using the DDPG algorithm. Next, we detail the modules in the algorithm.

\subsubsection{Pre-training procedure}
The agent applies the action $a_t$ selected by the actor network within the state $s_t$ to the environment in order to store the inputs of the environment ($a_t$ selected in $s_t$) and its outputs ($s^\prime_t$, $r_t$, and $d_t$) that constitute the transition $t$ in the replay buffer (cf. Figure~\ref{Rl_algo}). The training of the actor and critic networks can only begin once the replay buffer contains enough transitions to extract a batch. A batch is composed of elements (i.e., actions $a$, states $s$, next states $s^\prime$, etc.) coming from several non-sequential transitions. These transitions are selected randomly.

\subsubsection{Training procedure}
Making the agent learn from previous memories, i.e., using batches, accelerates learning and breaks undesirable temporal correlations\cite{Liu2018AACCCC}. The training of the critic network consists of reducing the error between the Q-values calculated using the Bellman equation $Q_B(s,a)$ (cf. (\ref{bellman_equation})) and the Q-values estimated by the critic network $Q(s,a)$ (cf. Figure~\ref{Rl_algo}). The Q-values number equals the batch size $N$, i.e., the number of selected transitions to train the agent. The Mean Square Error (MSE) optimization technique is used to reduce that error, i.e., we use the following Critic loss:
\begin{equation}
    \text{Critic loss} = \text{MSE}(Q_B(s,a),Q(s,a)).
\end{equation}

The weights of the critic network are updated based on the Critic loss. The ADAM optimizer\cite{Kingma2014ADAM} is used to calculate the gradient descent. The Q-values given by the critic network $Q(s,a)$ are used to evaluate the actions $a$ chosen by the actor at states $s$. Then, the actor's training is based on the Q-value given by the critic network, i.e., the actor loss is equal to the Q-value. Since the agent's training is made from a batch, one obtains as many Q-values $Q(s,a)$ (cf. Figure~\ref{Rl_algo}) as there are transitions in the batch. The policy loss is calculated by taking an average of the $Q(s,a)$ \cite{Lillicrap2015DDPG}:
%\vspace{-2 mm}
\begin{equation}\label{MSE}
    \text{Policy loss} = -\overline{Q(s,a)} = - \frac{\sum_{t=1}^{N} Q_t(s_t,a_t)}{N}.
\end{equation}
The weights of the actor network are updated based on the policy loss.

\subsubsection{Target networks}
Using a target network is a technique to stabilize learning. A target network is a copy of the main network's weights held constant to act as a stable target for learning for a fixed number of timesteps\cite{Lillicrap2015DDPG}. We use Polyak averaging to update the target networks (also called soft updating) once per the main network's update\cite{Sehgal2019ICR}:
\vspace{-1mm}
\begin{equation}% actor target network update
    W_{A_T} = \tau W_A + (1-\tau) W_{A_T}
\end{equation}
\vspace{-6mm}
\begin{equation}% critic target network update
    W_{C_T} = \tau W_C + (1-\tau) W_{C_T},
\end{equation}
where the used terms are:
\begin{itemize}
    \item $W_{A_T}$: the weights of the actor target network.
    \item $W_A$: the weights of the actor network.
    \item $W_{C_T}$: the weights of the critic target network.
    \item $W_C$: the weights of the critic network.
    \item $\tau$: the Polyak factor.
\end{itemize}

We choose to utilize the DDPG algorithm as our DRL algorithm because it is suitable for continuous action spaces. It has fewer parameters to set than other actor-critic DRL algorithms. It is a powerful tool to generalize the training, combined with parallel learning.

\subsection{Reward function}
The reward function is the key element that allows us to control and optimize the agent policy of choosing actions\cite{Zakaria2021Frontiers}. More details about choosing the suitable reward function are given in \cite{Sutton2018MIT, Plappert2018arXiv}. The simplest dense reward function for our task is to use a Euclidean distance-based calculation\cite{Laezza2021ICRA}. Therefore, our reward $r_t$ is calculated as the average Euclidean distance between the current positions of the selected mesh nodes, and their desired positions.

%We calculate the reward $r_t$ as the average Euclidean distance $D_t$ between the current positions of the selected mesh nodes to track $P_c$ and their desired positions $P_d$ (cf. (\ref{ShapedReward})). The number of selected mesh nodes to track is denoted by $m$, and a single mesh node is represented by $i$.

\subsection{Learning parallelization} \label{parallelization}
The actor-critic DRL algorithm A3C\cite{Mnih2016A3C} proposes to asynchronously execute multiple agents in parallel on various instances of the environment. That parallelism decorrelates the agent learning data since, at any transition, the parallel agents will be experiencing a variety of different states. Combining batch extraction and learning parallelization for off-policy algorithms ensures that the training data are decorrelated and can be collected faster\cite{Kretchmar2002CSCI, Clemente2017arXiv}. Thus, combining both techniques improves the overall learning time while achieving a better result from the generalization point of view. That is why we train the agent using DPPG on a single multi-core CPU, as in \cite{Mnih2016A3C}.



\section{Framework Implementation} \label{Methods}
After having introduced all the necessary DRL components, we describe how we apply them in our novel framework to address the specific problem scenario considered (Section \ref{sec_problem_statement}). We provide the implementation details including all assigned values for the DDPG and simulation parameters.

%\subsection{Problem statement}
%We propose a generalizable architecture to control the object's shape while the robot manipulates it. For simplicity, the robot grasps one end of the object, and the other is fixed to the ground. We describe the object's deformation by selecting some mesh nodes to track and record their position after deformation. 

\subsection{Framework overview}
Before starting the learning phase, we create a deformation space box within which the robot gripper tip moves to deform the object, and we record the positions of the selected nodes $P_d$ in a database. The reason for using a deformation space box is to record several deformations within a limited space that is reachable by the gripper tip. We have created two databases, each based on a box of different size: the training one, which is smaller, and the testing one, which is larger. All the details about the databases are mentioned in Section~\ref{sim_params}. The robot's objective is to manipulate the object so that the current positions of the selected nodes $P_c$ reach the desired positions $P_d$ within a tolerance threshold.

Figure~\ref{Rl_algo} gives an overview of our architecture. The action $a_t$ given by the DDPG to the agent (i.e., the robot) is the Cartesian velocity of the gripper tip $a_t \in \mathcal{A} = (V_x, V_y, V_z) \implies a_t \in \mathbb{R}^3$. The action $a_t$ is continuous since each element of the velocity ($V_x, V_y, \text{ or } V_z$) can have any value within the interval $ [-1,1]$. Then, the action $a_t$ is integrated according to the timestep (which is equal to \mbox{0.06 s}) to calculate the new gripper tip position $(X_n, Y_n, Z_n)$. The classical position-based controller available in Bullet moves the arm from its current position $(X_c,Y_c,Z_c)$ to the new one $(X_n,Y_n,Z_n)$.

The state $s_t \in \mathcal{S}$ is made up of the gripper tip current state $s_{g_t} \in \mathbb{R}^6$ and the current object shape $s_{o_t} \in \mathbb{R}^{6m}$ (cf. (\ref{state})) with $m$ the number of selected mesh nodes. $s_{g_t}$ includes the gripper tip position $(X_c,Y_c,Z_c)$ and velocity $(V_x, V_y, V_z)$. $s_{o_t}$ is composed of the positions of the selected mesh nodes $P_c \in \mathbb{R}^{3m}$, and their desired positions $P_d \in \mathbb{R}^{3m}$.
\begin{equation}\label{state}
    s_t = (s_{g_t}, s_{o_t}) \in \mathcal{S} = (X_c,Y_c,Z_c, V_x, V_y, V_z, P_c,  P_d).
\end{equation}
We calculate the reward $r_t$ as the average Euclidean distance $D_t$ between the current positions of the selected mesh nodes $P_c$ and their desired positions $P_d$ (cf. (\ref{ShapedReward})). Using subindex $i$ to denote the position of a single mesh node, we have:
\begin{equation} \label{ShapedReward} %https://en.wikipedia.org/wiki/Euclidean_distance
    r_t = -\overline{D_t(P_c,P_d)} = - \frac{\sum_{i=1}^{m} D_t(P_{c_i},P_{d_i})}{m}.
\end{equation}

\subsection{DDPG parameters}
The actor, actor target, critic, and critic target Deep Neural Networks (DNNs) have the same architecture: 3 Fully Connected (FC) hidden layers, each of which comprises 256 neurons. We use the Rectified Linear Unit (ReLU) as an activation function. We apply the Tanh function on the actor outputs $a_t$ to ensure that the gripper tip velocities remain in the interval $[-1,1]$. We add noise to the action $a_t$ using Ornstein–Uhlenbeck noise\cite{Lillicrap2015DDPG} for the exploration. We initialize the DNNs of the actor and critic with random values as in \cite{Lillicrap2015DDPG}. The actor target and critic target DNNs weights copy those of the actor and critic DNNs. The ADAM optimizer is used for gradient updates with learning rates of $\alpha_A = 0.0001$ for the actor and $\alpha_C = 0.001$ for the critic. A batch of 128 transitions is randomly sampled from the replay buffer, containing 50000 transitions. We use a constant discount factor $\gamma = 0.99$ and a constant Polyak factor $\tau = 0.01$.

Since we use parallel learning, in each episode, 32 agents are trying to achieve a different deformation during 300 transitions. This means that each agent makes 300 actions and passes through 300 different transitions to try to achieve 32 different goals (each agent has a different goal). Each action will have a reward $r_t$, and each agent will have a global reward equal to the sum of the action reward over the 300 transitions. This leads to having different gradients that are synchronized among the 32 agents, i.e., there will be one final gradient equal to the sum of all the 32 gradients. Then 32 agents networks are updated based on that final gradient so that all these networks keep having the same updated weights. We train the 32 agents during 63 episodes, which are equivalent to $32*63 = 2016$ episodes if we use a single agent and do not parallelize the training. The training lasts from 1000 to 1 million episodes in the literature\cite{Jangir2020ICRA, Laezza2021ICRA}. For training 32 agents, we used 32 CPU cores and the Python library MPI\cite{Dalcin2021MPI}. All the conducted training lasted less than three and a half hours.

\subsection{Simulation parameters}\label{sim_params}
We use PyBullet as physics engine of the simulator to train our agent. The simulator's physics engine uses the FEM method to simulate the soft object. The model of our soft object is built up from a 3D tetrahedral mesh. That model comprises 200 nodes, 392 tetrahedrons, 789 links, and 396 faces. The soft object has the following mechanical parameters: the Young's modulus is equal to 2.5 MPa, the Poisson coefficient is equal to 0.3, the mass is equal to 0.2 Kg, the damping ratio is equal to 0.01, and the friction coefficient is equal to 0.5. The simulation timestep is equal to 0.003 s. Note that we chose the timestep to integrate the action $a_t$ as equal to $20*0.003=0.06$ s., i.e., sufficiently larger than the simulation timestep.

We created two databases, each based on a box of different 3D size. The gripper tip moves inside that box to deform the object, and we recorded those deformations to use them as desired positions $P_d$ in the training and the testing phase. Figure~\ref{Deformation_box} shows the small and the large boxes. The small box size is equal to: 0.15 m on the x-axis, 0.5 m on the y-axis, and 0.25 m on the z-axis. The large box size is equal to: 0.2 m on the x-axis, 0.8 m on the y-axis, and 0.3 m on the z-axis. The small box is used to generate the small database, which contains 930 deformations. The large box is used to generate the large database, which includes 2651 deformations. The small database is used for the training, and both databases are used for the testing.

%\vspace{4 mm}

\begin{figure}[ht]
    \centering
    \includegraphics[width=8cm]{figures/RAL_Deformation_box.png}
    %\vspace{-2mm}
    \caption{The left plot presents the small box (in red) used to generate the small database. The right plot shows the large box (in red) used to generate the large database.}
    \label{Deformation_box}
    \vspace{-6mm}
\end{figure}


==> related_work_old.tex <==
\section{Related Work (TBD)}
